Incentivizing High Quality Crowdwork

We study the causal effects of financial incentives on the quality of crowdwork. We focus on performance-based payments (PBPs), bonus payments awarded to workers for producing high quality work. We design and run randomized behavioral experiments on the popular crowdsourcing platform Amazon Mechanical Turk with the goal of understanding when, where, and why PBPs help, identifying properties of the payment, payment structure, and the task itself that make them most effective. We provide examples of tasks for which PBPs do improve quality. For such tasks, the effectiveness of PBPs is not too sensitive to the threshold for quality required to receive the bonus, while the magnitude of the bonus must be large enough to make the reward salient. We also present examples of tasks for which PBPs do not improve quality. Our results suggest that for PBPs to improve quality, the task must be effort-responsive: the task must allow workers to produce higher quality work by exerting more effort. We also give a simple method to determine if a task is effort-responsive a priori. Furthermore, our experiments suggest that all payments on Mechanical Turk are, to some degree, implicitly performance-based in that workers believe their work may be rejected if their performance is sufficiently poor. Finally, we propose a new model of worker behavior that extends the standard principal-agent model from economics to include a worker's subjective beliefs about his likelihood of being paid, and show that the predictions of this model are in line with our experimental findings. This model may be useful as a foundation for theoretical studies of incentives in crowdsourcing markets.

==> setup.tex <==
\subsection{Tasks}

\begin{itemize}
	\item Proofreaing
	\item Spot the difference
	\item Handwriting recognition
	\item Audio transcription
\end{itemize}

\subsection{Randomized Treatments}

Randomly assigning workers to different treatments is key for our casual inference. In this work, we adopt two different methods of randomization as described below.

\subsubsection{Worker arrival sequence}

Before accepting the HIT, workers will first see a preview of the task and the base payment for this task. This preview and base payment is the same for all workers. 

After workers accept the HIT, we will then randomly assign them to different treatments. The randomization process is described as follows. Assume there are $K$ different treatments.

\begin{enumerate}
	\item Create a shuffled sequence from $1$ to $K$.
    \item Each arriving worker is assigned to the treatment in the shuffled sequence according to their arriving order.
    \item Re-shuffle the sequence for every $K$ worker arrivals.
\end{enumerate}

We have maintained an external server to deal with the randomization.

\xhdr{Benefits and Drawbacks}

The main benefit of this randomization process is that we can assign (almost) the same number of workers to each treatment.  

However, there are drawbacks too. First, since we will only explain the different payment rules after workers accept the HIT, workers in the control group are more likely to drop out the experiment since they don't have the bonus. Second, in the treatment with bonuses, since we announce the bonus after workers accept the HIT, this might create the reciprocity effects (i.e., workers are willing to exert more efforts since we are treating them nicely) and make the interpretation of our results more complicated.


\subsubsection{Recruiting a panel of workers}

We also adopt a different randomization strategy. We first post a recruiting HIT to recruit workers.  In this HIT, workers will be paid a small amount (5 cents) if they agree that we can send them up to three notifications about future tasks some time in the next month.  We are making it clear in the task description that they are under no obligation to do the future tasks, only to receive the notifications

After the recruitment, we obtain a list of workers' IDs we can send notifications. We randomly assign these workers to different treatment groups. We can then send notification emails to workers with a link to the treatment tasks they are assigned to.

To avoid workers seeing the task content of the treatments outside of their groups, we assign qualifications to workers and make sure only workers in the treatment can see the task content.

\xhdr{Benefits and Drawbacks}

The main benefit of this randomization process is that we can avoid workers anchoring their expectation (on payments or task difficulty) on the preview of the task.


